Omnigrasp: Grasping Diverse Objects with Simulated Humanoids

We present a method for controlling a simulated humanoid to grasp an object and move it to follow an object's trajectory. Due to the challenges in controlling a humanoid with dexterous hands, prior methods often use a disembodied hand and only consider vertical lifts or short trajectories. This limited scope hampers their applicability for object manipulation required for animation and simulation. To close this gap, we learn a controller that can pick up a large number (>1200) of objects and carry them to follow randomly generated trajectories. Our key insight is to leverage a humanoid motion representation that provides human-like motor skills and significantly speeds up training. Using only simplistic reward, state, and object representations, our method shows favorable scalability on diverse objects and trajectories. For training, we do not need a dataset of paired full-body motion and object trajectories. At test time, we only require the object mesh and desired trajectories for grasping and transporting. To demonstrate the capabilities of our method, we show state-of-the-art success rates in following object trajectories and generalizing to unseen objects. Code and models will be released.

==> assets/figures/supp_divserse.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=\textwidth]{assets/graphics/supp_diverse.jpeg}
\end{center}
   \caption{\small   $\name$  uses diverse strategies to grasp objects of different shapes. }
\label{fig:supp_diverse}

\end{figure}

==> assets/figures/teaser.tex <==
\begin{center}
    \centering
    \includegraphics[width=1\textwidth]{assets/graphics/teaser.jpeg}
    \captionof{figure}{\footnotesize{}}
    \label{fig:teaser}
\end{center}%


==> assets/tables/rebuttal_baselines.tex <==
\begin{table*}[t]

\centering
\caption{\small{Additional baselines on object grasp and trajectory following on the GRAB dataset. ``Traj'' indicates where the training object trajectory comes from. PHC (Row 1) uses ground-truth body motion as input. PPO-10B (Row 2) is training using RL without PULSE-X for a month ($\sim$10 billion samples). }} 
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|r|rrrrrrr|rrrrrrrr}
\toprule
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} &\multicolumn{7}{c}{GRAB-Goal-Test (Cross-Object, 140 sequences, 5 unseen objects)} & \multicolumn{7}{c}{GRAB-IMoS-Test (Cross-Subject, 92 sequences, 44 objects)} 
\\ 
\midrule
Method  & Traj & $\successgrasp \uparrow$  &  $\successtraj \uparrow$  &  $\ttr \uparrow$  & $\poserror  \downarrow$ &  $ \roterror \downarrow $ &  $\text{E}_{\text{acc}} \downarrow$  & $\text{E}_{\text{vel}} \downarrow$ & $\successgrasp \uparrow$ & $\successtraj \uparrow$ & $\ttr \uparrow$ & $\poserror  \downarrow$ &  $ \roterror \downarrow $ &  $\text{E}_{\text{acc}} \downarrow$  & $\text{E}_{\text{vel}} \downarrow$  \\ \midrule


PHC \cite{Luo2023-ft} & MoCap & 3.6\% & 11.4\% & 81.1\% & 66.3 & 0.8 & 1.5 & 3.8  & 0\% & 3.3\% & 97.4\% & 56.5 & {0.3} & {1.4} & {2.9}\\
\midrule 

PPO-10B  & Gen & { 98.4\%} & {55.9\%} & {97.5\%}  & {36.4} & \textbf{0.4} & {21.0} & {14.5} & {96.8\%}  & {53.2\%} & {97.9\%} & {35.6} & \textbf{0.5} & {19.6} & {13.9}  \\

AMP \cite{Peng2021-xu} & Gen & 90.4\% & 46.6\% & 94.0 \% & 40.7 & 0.6 & 5.3 & 5.3 & 95.8 \% & 49.2\% & 96.5\% & 34.9 & \textbf{0.5} & 6.2 & 6.0  \\

Braun \etal \cite{braun2023physically}  & MoCap &{79\%}  & {-} & { 85\%} & {-} & {-}  & {-}  & {- }  & { 64\%} & {-}  & {65\%} & {-}  & {-} & {-} &  {-} \\


\name  & MoCap &{94.6\%} & {84.8\% }  &  { 98.7\%}& \textbf{28.0} & {0.5} & \textbf{4.2}  & \textbf{4.3}    & {95.8\%}   & {85.4\%} & \textbf{99.8\%} & \textbf{27.5} & {0.6}  & \textbf{5.0} & \textbf{5.0} &  \\

\name  & Gen &{\textbf{100}\%}   & \textbf{94.1\% }& \textbf{99.6\%} & {30.2} & {0.93} & {5.4}  & {4.7}  & \textbf{ 98.9\%} & \textbf{90.5\%} & \textbf{99.8\%}  & {27.9} & {0.97}  & {6.3} & {5.4}  \\



% \text{Ours}   &  { \%} & {} & {}  & {} & {} & { \%} & {} & {}  & {} & {} & {\%} & {} & {} & {} & {}\\
\bottomrule 
\end{tabular}}
\label{tab:grab}


\end{table*}

